Retrieval-Augmented Data Augmentation for Low-Resource Domain Tasks

Despite large successes of recent language models on diverse tasks, they suffer from severe performance degeneration in low-resource settings with limited training data available. Many existing works tackle this problem by generating synthetic data from the training data and then training models on them, recently using Large Language Models (LLMs). However, in low-resource settings, the amount of seed data samples to use for data augmentation is very small, which makes generated samples suboptimal and less diverse. To tackle this challenge, we propose a novel method that augments training data by incorporating a wealth of examples from other datasets, along with the given training data. Specifically, we first retrieve the relevant instances from other datasets, such as their input-output pairs or contexts, based on their similarities with the given seed data, and then prompt LLMs to generate new samples with the contextual information within and across the original and retrieved samples. This approach can ensure that the generated data is not only relevant but also more diverse than what could be achieved using the limited seed data alone. We validate our proposed Retrieval-Augmented Data Augmentation (RADA) framework on multiple datasets under low-resource settings of training and test-time data augmentation scenarios, on which it outperforms existing LLM-powered data augmentation baselines.

==> Figures/analysis_embedding.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.99\columnwidth]{Figures/embedding_policyqa2.pdf}
    \vspace{-0.275in}
    \caption{Embedding Space on T-SNE}
    \label{fig:verify}
    \vspace{-0.125in}
\end{figure}

==> Figures/rouge_dist_all.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.975\linewidth]{Figures/tech_rouge.pdf}
    \vspace{-0.1in}
    \caption{\textbf{Distribution of the ROUGE-L scores} between generated data and seed data, with a set value of 30 on the Tech QA dataset.}
    \label{fig:concept}
    \vspace{-0.21in}
\end{figure*}

==> Figures/tsne_visualization.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.975\linewidth]{Figures/tsne_visualization_12.pdf}
    \vspace{-0.1in}
    \caption{\textbf{Embedding-space visualization results of samples} including the seed data and augmented data, using t-SNE. }
    \label{fig:tsne}
    \vspace{-0.21in}
\end{figure}



==> Tables/ablation.tex <==
\begin{table}[t!]
\caption{\textbf{Ablation studies} were conducted on the Tech QA dataset, employing Llama-7B-Chat as the data generator with seed data is 30 and augment 3,000\%. We focus on evaluating the effects of removing either the retriever or the filtering component.}
\vspace{-0.1in}
\label{tab:sensitivity}
\small
\centering
\resizebox{0.48\textwidth}{!}{
% \renewcommand{\arraystretch}{1.1}
% \renewcommand{\tabcolsep}{2.0mm}
\begin{tabular}{lc}
\toprule

%  & \textbf{71.33}& 70.26& 70.55 & 69.14& 71.22
\textbf{Methods} & \textbf{Tech QA}  \\

\midrule
\midrule

\textbf{Ours} & \textbf{44.37} \\

w/o In-context Retriever & 41.24  \\
w/o Target-context Retriever & 34.42 \\
w/o All Retriever & 30.38  \\
w/o Filtering & 42.43  \\

\bottomrule

\end{tabular}
}
\vspace{-0.05in}
\end{table}

==> Tables/main_results_llama.tex <==
 
\begin{table*}[t!]
\caption{\textbf{Train Time results on open-domain question answering} for Covid QA,Policy QA, Tech QA and Trivia QA with T5-Base of different seed data number 10, 30, 100 trained on generated by Llama-7B Chat. We emphasize the best results in bold.}
\vspace{-0.1in}
\label{tab:main}
\small
\centering
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{lcccccccccccc}
\toprule

 & \multicolumn{3}{c}{\bf Covid QA} & \multicolumn{3}{c}{\bf Policy QA } & \multicolumn{3}{c}{\bf Tech QA } & \multicolumn{3}{c}{\bf Average per Datasets } \\
\cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7} \cmidrule(l{2pt}r{2pt}){8-10} \cmidrule(l{2pt}r{2pt}){11-13} 
\textbf{Methods} & 10 & 30 & 100 & 10 & 30 & 100 & 10 & 30 & 100 & 10 & 30 & 100\\

\midrule
\midrule

% \multirowcell{5}[-0.5ex][l]{\textbf{Llama} } 
% \textbf{Llama} \\

Zero-shot & 12.79 & & & 8.02 & & & 26.18 \\

3-shot & 16.43 & & & 8.29 & & & 25.51 \\

Seed Data & 39.84 & 54.92 & 58.16 & 19.53 & 14.37 & 23.28 & 30.63 & 37.93 & 44.22 \\
\noalign{\vskip 0.25ex}\cdashline{1-13}\noalign{\vskip 0.75ex}

% Seed+External Data &  \\

Self-Instruct & 57.36 & 54.07 & & 14.71 & 20.98 & & 30.51 & 28.49 & &  \\

Original Data & 51.61 & 51.16 & & 18.76 & 19.50 & & 18.52 & 14.15 & & \\


Synthetic C,Q,A & 55.28 & 54.33 & & 22.02 & 18.86 & 13.78 & 26.56 & 30.85 & &\\

Synthetic Q,A & 45.01 & 43.07 & & 6.13 & 6.35 & & 15.04 & 31.39 & 15.13 &  \\

 \noalign{\vskip 0.25ex}\cdashline{1-13}\noalign{\vskip 0.75ex}

\textbf{Ours} & 52.35 & 45.08 & & 19.37 & 9.30 & 12.75 & 23.44 & 21.9 \\

\bottomrule

\end{tabular}
}
\vspace{-0.125in}
\end{table*}

==> Tables/retrieve_domains.tex <==
\begin{table}[t!]
\caption{\textbf{Analysis of domain adaptation on the retriever}, where we change the constrained domain pool of the retriever across two domain-specific QA benchmark datasets with seed data is 10 and augmented 3000\%.}
\vspace{-0.1in}
\label{tab:sensitivity}
\small
\centering
\resizebox{0.48\textwidth}{!}{
% \renewcommand{\arraystretch}{1.1}
% \renewcommand{\tabcolsep}{2.0mm}
\begin{tabular}{lcc}
\toprule

Domains & \textbf{Covid QA} & \textbf{Tech QA} \\

\midrule
\midrule

NQ+Domain Specific QA & 67.49 & 40.81 \\
\noalign{\vskip 0.25ex}\cdashline{1-3}\noalign{\vskip 0.75ex}

Biomedical & \textbf{67.75} & 40.09 \\
Computing & 66.70 & \textbf{42.67} \\

\bottomrule

\end{tabular}
}
\vspace{-0.05in}
\end{table}
